H.E.S.S. follow-up of BBH merger events

We present here, follow-up observations of four Binary black hole BBH events performed with the High Energy Stereoscopic System (H.E.S.S.) in the Very High Energy (VHE) gamma-ray domain during the second and third LIGO/Virgo observation runs. Detailed analyses of the obtained data did not show significant VHE emission. We derive integral upper limit maps considering a generic $E^{-2}$ source spectrum in the most sensitive H.E.S.S energy interval ranging from 1 to 10 TeV. We also consider Extragalactic Background Light absorption effects and derive integral upper limits over the full accessible energy range. We finally derive upper limits of the VHE luminosity for each event and compare them with the expected VHE emission from GRBs. These comparisons allow us to assess the H.E.S.S. gravitational wave follow-up strategies. For the fourth GW observing run O4, we do not expect to fundamentally alter our observing strategy, and will continue to prioritize sky coverage like for the previous runs

==> authors_ALL.tex <==
\author{H.E.S.S. Collaboration}
\author{H.~Abdalla}^{UNAM}
\author{F.~Aharonian}^{DIAS},\ref{MPIK},\ref{RAU}
\author{F.~Ait~Benkhali}^{MPIK}
\author{E.O.~Ang\"uner}^{CPPM}
\author{C.~Arcaro}^{NWU}
\author{C.~Armand}^{LAPP}
\author{T.~Armstrong}^{Oxford}
\author{H.~Ashkar}^{CEA}
\author{M.~Backes}^{UNAM,NWU}
\author{V.~Baghmanyan}^{IFJPAN}
\author{V.~Barbosa~Martins}^{DESY}
\author{A.~Barnacka}^{UJK}
\author{M.~Barnard}^{NWU}
\author{R.~Batzofin}^{Wits}
\author{Y.~Becherini}^{Linnaeus}
\author{D.~Berge}^{DESY}
\author{K.~Bernl\"ohr}^{MPIK}
\author{B.~Bi}^{IAAT}
\author{M.~B\"ottcher}^{NWU}
\author{C.~Boisson}^{LUTH}
\author{J.~Bolmont}^{LPNHE}
\author{M.~de~Bony~de~Lavergne}^{LAPP}
\author{M.~Breuhaus}^{MPIK}
\author{R.~Brose}^{DIAS}
\author{F.~Brun}^{CEA}
\author{T.~Bulik}^{UWarsaw}
\author{T.~Bylund}^{Linnaeus}
\author{F.~Cangemi}^{LPNHE}
\author{S.~Caroff}^{LPNHE}
\author{S.~Casanova}^{IFJPAN}
\author{J.~Catalano}^{ECAP}
\author{P.~Chambery}^{CENBG}
\author{T.~Chand}^{NWU}
\author{A.~Chen}^{Wits}
\author{G.~Cotter}^{Oxford}
\author{M.~Cury{\l}o}^{UWarsaw}
\author{J.~Damascene~Mbarubucyeye}^{DESY}
\author{I.D.~Davids}^{UNAM}
\author{J.~Davies}^{Oxford}
\author{J.~Devin}^{CENBG}
\author{A.~Djannati-Ata\"i}^{APC}
\author{A.~Dmytriiev}^{LUTH}
\author{A.~Donath}^{MPIK}
\author{V.~Doroshenko}^{IAAT}
\author{L.~Dreyer}^{NWU}
\author{L.~Du~Plessis}^{NWU}
\author{C.~Duffy}^{Leicester}
\author{K.~Egberts}^{UP}
\author{S.~Einecke}^{Adelaide}
\author{}^{LPNHE}
\author{J.-P.~Ernenwein}^{CPPM}
\author{S.~Fegan}^{LLR}
\author{K.~Feijen}^{Adelaide}
\author{A.~Fiasson}^{LAPP}
\author{G.~Fichet~de~Clairfontaine}^{LUTH}
\author{G.~Fontaine}^{LLR}
\author{F.~Lott}^{UNAM}
\author{M.~F\"u{\ss}ling}^{DESY}
\author{S.~Funk}^{ECAP}
\author{S.~Gabici}^{APC}
\author{Y.A.~Gallant}^{LUPM}
\author{}^{LSW}
\author{G.~Giavitto}^{DESY}
\author{L.~Giunti}^{APC,{CEA}
\author{D.~Glawion}^{ECAP}
\author{J.F.~Glicenstein}^{CEA}
\author{M.-H.~Grondin}^{CENBG}
\author{S.~Hattingh}^{NWU}
\author{M.~Haupt}^{DESY}
\author{G.~Hermann}^{MPIK}
\author{J.A.~Hinton}^{MPIK}
\author{W.~Hofmann}^{MPIK}
\author{C.~Hoischen}^{UP}
\author{T.~L.~Holch}^{DESY}
\author{M.~Holler}^{Innsbruck}
\author{D.~Horns}^{UHH}
\author{Zhiqiu~Huang}^{MPIK}
\author{D.~Huber}^{Innsbruck}
\author{M.~H\"{o}rbe}^{Oxford}
\author{M.~Jamrozy}^{UJK}
\author{F.~Jankowsky}^{LSW}
\author{V.~Joshi}^{ECAP}
\author{I.~Jung-Richardt}^{ECAP}
\author{E.~Kasai}^{UNAM}
\author{K.~Katarzy{\'n}ski}^{NCUT}
\author{U.~Katz}^{ECAP}
\author{D.~Khangulyan}^{Rikkyo}
\author{B.~Kh\'elifi}^{APC}
\author{S.~Klepser}^{DESY}
\author{W.~Klu\'{z}niak}^{NCAC}
\author{Nu.~Komin}^{Wits}
\author{R.~Konno}^{DESY}
\author{K.~Kosack}^{CEA}
\author{D.~Kostunin}^{DESY}
\author{M.~Kreter}^{NWU}
\author{G.~Kukec~Mezek}^{Linnaeus}
\author{A.~Kundu}^{NWU}
\author{G.~Lamanna}^{LAPP}
\author{S.~Le Stum}^{CPPM}
\author{A.~Lemi\`ere}^{APC}
\author{M.~Lemoine-Goumard}^{CENBG}
\author{J.-P.~Lenain}^{LPNHE}
\author{F.~Leuschner}^{IAAT}
\author{C.~Levy}^{LPNHE}
\author{T.~Lohse}^{HUB}
\author{A.~Luashvili}^{LUTH}
\author{I.~Lypova}^{LSW}
\author{J.~Mackey}^{DIAS}
\author{J.~Majumdar}^{DESY}
\author{D.~Malyshev}^{IAAT}
\author{D.~Malyshev}^{ECAP}
\author{V.~Marandon}^{MPIK}
\author{P.~Marchegiani}^{Wits}
\author{A.~Marcowith}^{LUPM}
\author{A.~Mares}^{CENBG}
\author{G.~Mart\'i-Devesa}^{Innsbruck}
\author{R.~Marx}^{LSW}
\author{G.~Maurin}^{LAPP}
\author{P.J.~Meintjes}^{UFS}
\author{M.~Meyer}^{ECAP}
\author{A.~Mitchell}^{MPIK}
\author{R.~Moderski}^{NCAC}
\author{L.~Mohrmann}^{ECAP}
\author{A.~Montanari}^{CEA}
\author{C.~Moore}^{Leicester}
\author{}^{Oxford}
\author{E.~Moulin}^{CEA}
\author{J.~Muller}^{LLR}
\author{T.~Murach}^{DESY}
\author{K.~Nakashima}^{ECAP}
\author{M.~de~Naurois}^{LLR}
\author{A.~Nayerhoda}^{IFJPAN}
\author{H.~Ndiyavala}^{NWU}
\author{J.~Niemiec}^{IFJPAN}
\author{A.~Priyana~Noel}^{UJK}
\author{P.~O'Brien}^{Leicester}
\author{L.~Oberholzer}^{NWU}
\author{S.~Ohm}^{DESY}
\author{L.~Olivera-Nieto}^{MPIK}
\author{E.~de~Ona~Wilhelmi}^{DESY}
\author{M.~Ostrowski}^{UJK}
\author{S.~Panny}^{Innsbruck}
\author{M.~Panter}^{MPIK}
\author{R.D.~Parsons}^{HUB}
\author{G.~Peron}^{MPIK}
\author{S.~Pita}^{APC}
\author{V.~Poireau}^{LAPP}
\author{D.A.~Prokhorov}^{Amsterdam}
\author{H.~Prokoph}^{DESY}
\author{G.~P\"uhlhofer}^{IAAT}
\author{M.~Punch}^{APC,Linnaeus}
\author{A.~Quirrenbach}^{LSW}
\author{P.~Reichherzer}^{CEA}
\author{A.~Reimer}^{Innsbruck}
\author{O.~Reimer}^{Innsbruck}
\author{Q.~Remy}^{MPIK}
\author{M.~Renaud}^{LUPM}
\author{B.~Reville}^{MPIK}
\author{F.~Rieger}^{MPIK}
\author{C.~Romoli}^{MPIK}
\author{G.~Rowell}^{Adelaide}
\author{B.~Rudak}^{NCAC}
\author{H.~Rueda Ricarte}^{CEA}
\author{E.~Ruiz-Velasco}^{MPIK}
\author{V.~Sahakian}^{Yerevan}
\author{S.~Sailer}^{MPIK}
\author{H.~Salzmann}^{IAAT}
\author{D.A.~Sanchez}^{LAPP}
\author{A.~Santangelo}^{IAAT}
\author{M.~Sasaki}^{ECAP}
\author{J.~Sch\"afer}^{ECAP}
\author{H.M.~Schutte}^{NWU}
\author{U.~Schwanke}^{HUB}
\author{F.~Sch\"ussler}^{CEA}
\author{M.~Senniappan}^{Linnaeus}
\author{A.S.~Seyffert}^{NWU}
\author{J.N.S.~Shapopi}^{UNAM}
\author{K.~Shiningayamwe}^{UNAM}
\author{R.~Simoni}^{Amsterdam}
\author{A.~Sinha}^{LUPM}
\author{H.~Sol}^{LUTH}
\author{}^{Oxford}
\author{A.~Specovius}^{ECAP}
\author{S.~Spencer}^{Oxford}
\author{M.~Spir-Jacob}^{APC}
\author{{\L.}~Stawarz}^{UJK}
\author{R.~Steenkamp}^{UNAM}
\author{C.~Stegmann}^{UP,DESY}
\author{S.~Steinmassl}^{MPIK}
\author{C.~Steppa}^{UP}
\author{L.~Sun}^{Amsterdam}
\author{T.~Takahashi}^{Rikkyo}
\author{T.~Tanaka}^{Rikkyo}
\author{T.~Tavernier}^{CEA}
\author{A.M.~Taylor}^{DESY}
\author{R.~Terrier}^{APC}
\author{J.~H.E.~Thiersen}^{NWU}
\author{C.~Thorpe-Morgan}^{IAAT}
\author{M.~Tluczykont}^{UHH}
\author{L.~Tomankova}^{ECAP}
\author{M.~Tsirou}^{MPIK}
\author{N.~Tsuji}^{Rikkyo}
\author{R.~Tuffs}^{MPIK}
\author{Y.~Uchiyama}^{Rikkyo}
\author{D.J.~van~der~Walt}^{NWU}
\author{C.~van~Eldik}^{ECAP}
\author{C.~van~Rensburg}^{UNAM}
\author{B.~van~Soelen}^{UFS}
\author{G.~Vasileiadis}^{LUPM}
\author{J.~Veh}^{ECAP}
\author{C.~Venter}^{NWU}
\author{P.~Vincent}^{LPNHE}
\author{J.~Vink}^{Amsterdam}
\author{H.J.~V\"olk}^{MPIK}
\author{S.J.~Wagner}^{LSW}
\author{J.~Watson}^{Oxford}
\author{F.~Werner}^{MPIK}
\author{R.~White}^{MPIK}
\author{A.~Wierzcholska}^{IFJPAN}
\author{Yu~Wun~Wong}^{ECAP}
\author{H.~Yassin}^{NWU}
\author{A.~Yusafzai}^{ECAP}
\author{M.~Zacharias}^{LUTH}
\author{R.~Zanin}^{MPIK}
\author{D.~Zargaryan}^{DIAS,RAU}
\author{A.A.~Zdziarski}^{NCAC}
\author{A.~Zech}^{LUTH}
\author{S.J.~Zhu}^{DESY}
\author{A.~Zmija}^{ECAP}
\author{S.~Zouari}^{APC}
\author{N.~\.Zywucka}^{NWU}
}

\institute{
University of Namibia, Department of Physics, Private Bag 13301, Windhoek 10005, Namibia \label{UNAM} \and
Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, Dublin 2, Ireland \label{DIAS} \and
Max-Planck-Institut f\"ur Kernphysik, P.O. Box 103980, D 69029 Heidelberg, Germany \label{MPIK} \and
High Energy Astrophysics Laboratory, RAU,  123 Hovsep Emin St  Yerevan 0051, Armenia \label{RAU} \and
Aix Marseille Universit\'e, CNRS/IN2P3, CPPM, Marseille, France \label{CPPM} \and
Centre for Space Research, North-West University, Potchefstroom 2520, South Africa \label{NWU} \and
Laboratoire d'Annecy de Physique des Particules, Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS, LAPP, 74000 Annecy, France \label{LAPP} \and
University of Oxford, Department of Physics, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK \label{Oxford} \and
IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France \label{CEA} \and
Instytut Fizyki J\c{a}drowej PAN, ul. Radzikowskiego 152, 31-342 Krak{\'o}w, Poland \label{IFJPAN} \and
DESY, D-15738 Zeuthen, Germany \label{DESY} \and
Obserwatorium Astronomiczne, Uniwersytet Jagiello{\'n}ski, ul. Orla 171, 30-244 Krak{\'o}w, Poland \label{UJK} \and
School of Physics, University of the Witwatersrand, 1 Jan Smuts Avenue, Braamfontein, Johannesburg, 2050 South Africa \label{Wits} \and
Department of Physics and Electrical Engineering, Linnaeus University,  351 95 V\"axj\"o, Sweden \label{Linnaeus} \and
Institut f\"ur Astronomie und Astrophysik, Universit\"at T\"ubingen, Sand 1, D 72076 T\"ubingen, Germany \label{IAAT} \and
Laboratoire Univers et Théories, Observatoire de Paris, Université PSL, CNRS, Université de Paris, 92190 Meudon, France \label{LUTH} \and
Sorbonne Universit\'e, Universit\'e Paris Diderot, Sorbonne Paris Cit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies, LPNHE, 4 Place Jussieu, F-75252 Paris, France \label{LPNHE} \and
Astronomical Observatory, The University of Warsaw, Al. Ujazdowskie 4, 00-478 Warsaw, Poland \label{UWarsaw} \and
Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg, Erlangen Centre for Astroparticle Physics, Erwin-Rommel-Str. 1, D 91058 Erlangen, Germany \label{ECAP} \and
Universit\'e Bordeaux, CNRS/IN2P3, Centre d'\'Etudes Nucl\'eaires de Bordeaux Gradignan, 33175 Gradignan, France \label{CENBG} \and
Université de Paris, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France \label{APC} \and
Department of Physics and Astronomy, The University of Leicester, University Road, Leicester, LE1 7RH, United Kingdom \label{Leicester} \and
Institut f\"ur Physik und Astronomie, Universit\"at Potsdam,  Karl-Liebknecht-Strasse 24/25, D 14476 Potsdam, Germany \label{UP} \and
School of Physical Sciences, University of Adelaide, Adelaide 5005, Australia \label{Adelaide} \and
Laboratoire Leprince-Ringuet, École Polytechnique, CNRS, Institut Polytechnique de Paris, F-91128 Palaiseau, France \label{LLR} \and
Laboratoire Univers et Particules de Montpellier, Universit\'e Montpellier, CNRS/IN2P3,  CC 72, Place Eug\`ene Bataillon, F-34095 Montpellier Cedex 5, France \label{LUPM} \and
Landessternwarte, Universit\"at Heidelberg, K\"onigstuhl, D 69117 Heidelberg, Germany \label{LSW} \and
Institut f\"ur Astro- und Teilchenphysik, Leopold-Franzens-Universit\"at Innsbruck, A-6020 Innsbruck, Austria \label{Innsbruck} \and
Universit\"at Hamburg, Institut f\"ur Experimentalphysik, Luruper Chaussee 149, D 22761 Hamburg, Germany \label{UHH} \and
Institute of Astronomy, Faculty of Physics, Astronomy and Informatics, Nicolaus Copernicus University,  Grudziadzka 5, 87-100 Torun, Poland \label{NCUT} \and
Department of Physics, Rikkyo University, 3-34-1 Nishi-Ikebukuro, Toshima-ku, Tokyo 171-8501, Japan \label{Rikkyo} \and
Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, ul. Bartycka 18, 00-716 Warsaw, Poland \label{NCAC} \and
Institut f\"ur Physik, Humboldt-Universit\"at zu Berlin, Newtonstr. 15, D 12489 Berlin, Germany \label{HUB} \and
Department of Physics, University of the Free State,  PO Box 339, Bloemfontein 9300, South Africa \label{UFS} \and
GRAPPA, Anton Pannekoek Institute for Astronomy, University of Amsterdam,  Science Park 904, 1098 XH Amsterdam, The Netherlands \label{Amsterdam} \and
Yerevan Physics Institute, 2 Alikhanian Brothers St., 375036 Yerevan, Armenia \label{Yerevan}
}

